Rapidly Decaying Supernova 2010X: A Candidate ".Ia" Explosion

We present the discovery, photometric and spectroscopic follow-up observations of SN 2010X (PTF 10bhp). This supernova decays exponentially with tau_d=5 days, and rivals the current recordholder in speed, SN 2002bj. SN 2010X peaks at M_r=-17mag and has mean velocities of 10,000 km/s. Our light curve modeling suggests a radioactivity powered event and an ejecta mass of 0.16 Msun. If powered by Nickel, we show that the Nickel mass must be very small (0.02 Msun) and that the supernova quickly becomes optically thin to gamma-rays. Our spectral modeling suggests that SN 2010X and SN 2002bj have similar chemical compositions and that one of Aluminum or Helium is present. If Aluminum is present, we speculate that this may be an accretion induced collapse of an O-Ne-Mg white dwarf. If Helium is present, all observables of SN 2010X are consistent with being a thermonuclear Helium shell detonation on a white dwarf, a ".Ia" explosion. With the 1-day dynamic-cadence experiment on the Palomar Transient Factory, we expect to annually discover a few such events.

==> tabs.tex <==
\begin{deluxetable}{llll}[!hbt]
  \tabletypesize{\footnotesize}
  \tablecaption{Optical Light Curve}
  \tablecolumns{4}
  \tablewidth{0pc}
 \tablehead{\colhead{MJD} & \colhead{Filter} & \colhead{Mag} & \colhead{Facility}
}
 \startdata
      55207.3  &  r  &    $<$20.91          & Palomar 48-in  \\
      55207.4  &  r  &    $<$20.85          & Palomar 48-in  \\
      55213.2  &  r  &    $<$20.48          & Palomar 48-in  \\
      55221.2  &  r  &    $<$20.42          & Palomar 48-in  \\
      55234.1  &  r  &    17.95 $\pm$ 0.15  & Rich           \\
      55237.1  &  r  &    17.43 $\pm$ 0.12  & Rich           \\
      55239.2  &  r  &    17.41 $\pm$ 0.19  & Brimacombe     \\ 
      55246.1  &  r  &    17.84 $\pm$ 0.09  & Palomar 48-in  \\
      55246.2  &  r  &    17.79 $\pm$ 0.10  & Palomar 48-in  \\
      55246.3  &  r  &    17.78 $\pm$ 0.09  & Palomar 48-in  \\
      55246.3  &  r  &    17.83 $\pm$ 0.09  & Palomar 48-in  \\
      55251.1  &  r  &    18.77 $\pm$ 0.12  & Palomar 48-in  \\
      55251.3  &  g  &    19.61 $\pm$ 0.18  & LCOGT/FTN   \\
      55251.3  &  r  &    18.87 $\pm$ 0.10  & LCOGT/FTN   \\
      55251.3  &  i  &    18.74 $\pm$ 0.12  & LCOGT/FTN   \\
      55254.3  &  g  &    21.02 $\pm$ 0.34  & LCOGT/FTN   \\
      55254.3  &  r  &    19.74 $\pm$ 0.13  & LCOGT/FTN   \\
      55254.3  &  i  &    19.57 $\pm$ 0.14  & LCOGT/FTN   \\
      55255.3  &  r  &    19.96 $\pm$ 0.11  & LCOGT/FTN   \\
      55256.3  &  g  &    $<$20.66          & LCOGT/FTN   \\
      55256.3  &  i  &    20.39 $\pm$ 0.17  & LCOGT/FTN   \\    
      55268.1  &  r  &    $<$20.72          & Palomar 48-in \\
      55282.3  &  r  &    $<$20.70          & LCOGT/FTN   \\
      55294.1  &  r  &    $<$22.55          & Palomar 200-in  
 \enddata
\label{tab:lc}
\end{deluxetable}


